The Hausdorff dimension of the boundary of the Mandelbrot set and Julia sets

It is shown that the boundary of the Mandelbrot set $M$ has Hausdorff dimension two and that for a generic $c \in \bM$, the Julia set of $z \mapsto z^2+c$ also has Hausdorff dimension two. The proof is based on the study of the bifurcation of parabolic periodic points.

==> hdimBB.tex <==
\heading 
Appendix.  Proof of the properties of Ecalle cylinders 
\endheading 
\medskip 

To be added! 

In this Appendix, we give the proof or comments for the facts which were stated in 
\S4 and \S7.  Note that most of the facts in \S 4.1 are classical and 
can be found in [Mi].  
The facts in \S 4.2 can be found in Douady-Hubbard [DH] in a different form.   

\comment 
\subheading{\S\S 4.1--4.3} 

Most of facts are classical, see [Mi] for example.  Here are some comments.  
\newline 
(4.1.1) and (4.1.2) are straightforward by a computation and left to the reader.  
\newline 
For (4.2.1) and (4.2.2), see Proposition ?? and Lemma ?? below.  
\newline 
(4.2.3) follows from (4.2.2) via a simple computation.  
\newline 
(4.2.4) First note that $\Phi_-(\Q_- \cap \Q_+)$ contains 
$\{ z \bigm|\ |\Re z|<1, \ |\Im z|> \eta \}$ for some $\eta >0$, and that 
$\tE_{f_0}(z+1)=\tE_{f_0}(z)+1$ if both $z, z+1$ are in 
this set.  Then one can use this relation to extend $\tE_{f_0}$ to 
$\{z\bigm|\ |\Im z|> \eta\}$.  The rest follows easily.  
\newline 
(4.3.1) The property of the extension is immediate from the definition.  

\bigskip 

\subheading{General construction}  

Define for $b_1, b_2 \in \C$ with $\Re b_1 < \Re b_2$, 
$$ 
\Cal Q(b_1, b_2) =\{z \in \C| \ \Re (z-b_1)> -|\Im (z-b_1)|, \ 
\Re (z-b_2) < |\Im (z-b_2)|\ \}.  
$$
If $b_1=-\infty$ (resp. $b_2=\infty$), the condition involving 
$b_1$ (resp. $b_2$) should be removed.  



\proclaim{Proposition A.1} 
Let $F$ be a holomorphic function defined in $\Q=\Q(b_1,b_2)$, 
where $\Re b_2 > \Re b_1 +2$  (here $b_1$ or $b_2$ may be $-\infty$ or 
$\infty$).  Suppose 
$$|F(z)-(z+1)|< \frac14, \ \text{ and } |F'(z)-1| < \frac 14 
\ \text{ for } z \in \Q. \tag {5?}$$
Then
\newline
(0) $F$ is univalent on $\Q$.  
\newline
(i) Let $z_0 \in \Q$ be a point such that  $\Re b_1 < \Re z_0 <\Re b_2 -5/4$.  
Denote by $S$ the closed region (a strip) bounded by the two curves 
$\ell=\{z_0+iy| y \in \R\}$ and $F(\ell)$.  Then for any $z \in \Q$, 
there exists a unique $n \in \Z$ such that $F^n(w)$ is defined and 
belongs to $S-F(\ell)$.  
\newline
(ii) There exists a univalent function $\Phi : \Q\to \C$
satisfying 
$$\Phi(F(z))=\Phi(z) + 1 .$$
Moreover other such functions are written as $\Phi+constant$.  
\newline
(iii) If we normalize $\Phi$ by $\Phi(z_0)=0$, where $z_0 \in \Q$, 
then the correspondence $F \mapsto \Phi$ is continuous 
with respect to the compact-open topology.  (See also \S 4.0 Notations.)  
 
\endproclaim 

\demo{Proof}  
(0) and (i) are easy and left to the reader.  
\newline 
(ii) Let $z_0 \in \Q$ be as in (i).  
Define $h_1: \{z|\ 0 \leq \Re z \leq 1\} \to \Q $ by 
$$h_1(x+iy)=(1-x)(z_0+iy) + xF(z_0+iy) , \ \text{ for } 0\leq x\leq 1,\ y \in\R.$$
Then we have 
$$
\frac {\partial h_1}{\partial x}=F(z_0+iy)-(z_0+iy), \ 
\frac {\partial h_1}{\partial y}=ixF'(z_0+iy)+i(1-x).  
$$
Hence 
$$
\biggl|\frac {\partial h_1}{\partial z}-1 \biggr|
=\frac12 \bigl|\{F(z_0)-(z_0+iy+1)\}+x(F'(z_0+iy)-1)\bigr| \leq \frac 14, 
$$
$$
\biggl|\frac {\partial h_1}{\partial \bar z}\biggr|
=\frac12 \bigl|\{F(z_0)-(z_0+iy+1)\}-x(F'(z_0+iy)-1) \bigr| \leq \frac 14.  
$$ 
 
Therefore $\bigl| \frac {\partial h_1}{\partial \bar z}/
\frac {\partial h_1}{\partial z}\bigr|<1/3$ and 
$h_1$ is a quasiconformal mapping onto the strip $S$, and satisfies 
$h_1^{-1}(F(z))=h_1^{-1}(z)+1$  for  $ z \in \ell$.   
Let $\sigma_0$ be the standard conformal structure of $\C$, and take the 
pull-back $\sigma = h_1^*\sigma_0$ on $ \{z|\ 0 \leq \Re z \leq 1\}$.  
Then extend $\sigma$
to $\C$ by  $\sigma=(T^n)^* \sigma$ on $\{z| -n \leq \Re z \leq -n+1\}$, 
where $T(z)=z+1$ .  
By Ahlfors-Bers measurable mapping theorem [A], there exists a unique 
quasiconformal mapping $h_2:\C \to \C$ such that $h_2^*\sigma_0=\sigma$ 
and $h_2(0)=0, \ h_2(1)=1$.  By the definition of $\sigma$,  $T$ preserves 
$\sigma$.  Hence $h_2 \circ T \circ h_2^{-1}$ preserves the standard conformal 
structure $\sigma_0$, i.e. conformal, therefore it must be an affine function.  
Since  $T$  has no fixed point in $\C$, so does  $h_2 \circ T \circ h_2^{-1}$, 
hence it is a translation.  Using  $h_2 \circ T \circ h_2^{-1}(0)=1$, we 
have  $h_2 \circ T \circ h_2^{-1}=T$.  

  Now define $\Phi$ by 
$\Phi=h_2 \circ h_1^{-1} $ on $S$ , and extend to the whole $\Q$ using 
the relation 
$ \Phi(F(z))=\Phi(z)+1 .$
Then $\Phi$ is well-defined by (i), continuous and homeomorphic by the 
above relations on $h_1^{-1}$ and $h_2$.   
Moreover $\Phi$ is analytic outside the orbit of $\ell$, 
then analytic in the whole $\Q$ by Morera's theorem.  Thus we have obtained 
the desired univalent function $\Phi$.  


If $\Phi'$ is another such function, 
then $\Phi''(z)=\Phi' \circ \Phi^{-1}$ commutes with $T$ at least in $\Phi(\Q)$.  
Hence $\Phi''(z)-z$ extends to $\C$ as a periodic function, then $\Phi''$ extends 
to $\C$ as a holomorphic function commuting with $T$.  Similarly ${\Phi''}^{-1}$ 
also has this property, therefore $\phi$ must be an affine function.  However 
an affine function commuting with the translation $T$ is also a translation by 
a constant.  Hence the assertion follows.  

(iii) Let us consider $F$ and $F_0$ defined in the same $\Q$ and satisfying the 
condition of the Proposition.  As in (ii), 
we can construct $h_1$, $h_2$, $\Phi$ for $F$ and $h_{1,0}$, $h_{2,0}$, 
$\Phi_0$ for $F_0$.  
It is easy to see that on any compact set of $\{z| 0\leq \Re z \leq 1\}$, 
$\frac {\partial h_1}{\partial \bar z}/
\frac {\partial h_1}{\partial z} \to 
\frac {\partial h_{1,0}}{\partial \bar z}/
\frac {\partial h_{1,0}}{\partial z}$ 
as $F \to F_0$.   Hence 
$\sigma_F=h_1^* \sigma_0 \to \sigma_{F_0}=h_{1,0}^* \sigma_0$ and 
$h_2 \to h_{2,0}$ on any compact set as $f \to F_0$.  
It follows from the definition of the extension of $\Phi$ that 
$\Phi \to \Phi_0$ as $F \to F_0$.  
\qed \enddemo


  A strip $S$ as in Lemma 5. ??(i), is called a {\it fundamental region} 
for the map $F|_\Q$.  The quotient space 
$$\aligned 
\Cal C &=S/_\sim, \ \text{ where } \ell \ni z \sim F(z) \in F(\ell) \\ 
&= \Q/_\sim, \ \text{ where }  z \sim F(z) \text{ if } 
z \in \Q \cap F^{-1}(\Q)  
\endaligned $$
is topologically a cylinder which is called the {\it Ecalle cylinder}.  
Moreover, 
$\Cal C$ has a natural structure of a Riemann surface, using $F$ near $\ell$ 
as a coordinate patching.  \enddefinition 

In fact, 

\proclaim{Lemma} Let $F$, $\Q$, $S$ be as in Lemma 5.?  Then 
$\pi \circ \Phi$ induces an isomorphism 
$$\overline \Phi:\Cal C=S/_\sim  \to \C^*=\C-\{0\}.$$
\endproclaim
Proof.  Let $L$ be the component of $\C-\Phi(\ell)$ not containing 
$\Phi(F(\ell))$

\proclaim{Lemma (Some estimates)}
Suppose that $\Phi$ and $v$ are holomorphic 
functions in a region $\Cal U$ satisfying: 
$$\Phi \ \text{ is univalent in } \Cal U, \ \ 
|v(z)-1|<1/4 \ \text{ for } z \in \Cal U \ \text{ and }$$
$$\Phi(z+v(z))=\Phi(z)+1 , \ \text{  if }\ z, z+v(z) \in \Cal U.$$

(i)  There exist universal constants $R_1, C_1, C_2>0$  such that if 
$\Cal U=\{z \bigl| \ |z-z_0|<R\}$ for $R \geq R_1$, then 
$$ \bigl|\Phi'(z_0)-\frac 1{v(z_0)}\bigr| \leq 
C_1\left(\frac1{R^2}+|v'(z_0)|\right)
\leq \frac{C_2}{R} .  $$

(ii) Suppose $\Cal U=\{z \in \C^*| \ \theta_1< \arg z < \theta_2 \}$ 
$(\theta_2 < \theta_1+2 \pi)$ and $|a'(z)|\leq C/|z|^{1+\nu}$ $(z \in \Cal U)$ 
for some $C, \nu >0$.  For $z_0 \in \Cal U$ and $\theta'_1, \ \theta'_2$ 
with $\theta_1<\theta'_1<\theta'_2<\theta_2$, there exists $R_2, C_3>0$ and 
$\xi \in \C$ such that 
$$\bigl|\Phi(z)-\int_{z_0}^z \frac {d\zeta}{v(\zeta)}-\xi \bigr| \leq 
C_3\left(\frac 1{|z|}+\frac C{|z|^\nu}\right),$$
for $z$ satisfying $\theta'_1 < \arg z < \theta'_2$, $dist(z, \C-\Cal U)>R_1$.  
Moreover $C_3$ depend only on $\theta_i, \theta_i'$.  
\endproclaim

\demo{Proof} (i) We may suppose $z_0=0$.  
We take $R$ so that $R>> 1$.  
It follows from Koebe's distortion theorem [?] that if 
$|z|<R-2$, then 
$$
\frac{|v(z)|}{(1+|v(z)|/2)^2} \leq 
\biggl| \frac{\Phi(z+v(z))-\Phi(z)}{\Phi'(z)} \biggr| \leq 
\frac{|v(z)|}{(1-|v(z)|/2)^2},
$$
since $\Phi$ is univalent in $\{\zeta \bigl| \ |\zeta -z|<2\ \}$.   Hence 
$C \leq |\Phi'(z)| \leq C'$  if  $|z|<R-2$.  
We have 
$|\Phi''(z)|\leq C/R$  if $|z|<R/2$. 
(In fact, by Cauchy's formula, $\Phi''(z)$ can be expressed in terms of 
an integral of $\Phi'(\zeta)/(\zeta-z)^2$ over the contour 
$\{\zeta \bigl| \ |\zeta-z|=R/2\}$, then use the above estimate.)
Using the formula 
$$
\Phi(z+a)=\Phi(z)+a\Phi'(z)+a^2\int_0^1 (1-t)\Phi''(z+at)dt, 
$$
we obtain $|1-\Phi'(z)v(z)| \leq C/R$ if  $|z|<R/2-5/4$.  
Again by Cauchy's formula, 
$|(1-\Phi'(z)v(z))'|=|\Phi''(z)v(z)+\Phi'(z)v'(z)| \leq C/R^2$  
if $|z|<R/4$.  It also follows from Cauchy's formula that 
$|v''(z)|\leq C/R^2$ for $|z|<R/2$.  Hence we have 
$|\Phi''(z)| \leq C(1/R^2+|v'(0)|)$ for $|z|<R/4$.  By the above formula 
again, we have $|1-\Phi'(0)v(0)|\leq C(1/R^2+|v'(0)|)$.  



\subheading{A.3 Coordinate changes} 

  Let $f_0$ be as in \S 4.2.  Hence $f_0(z)=z+z^2+\dots$.  

\proclaim{Lemma 4.3}
There exist a neighbourhood $\N$ of $f_0$ in $\Cal F$ and $\rho >0$ 
such that if $f \in \N$ then $\overline D_\rho \subset \Dom(f)$ and 
$f(z)$ can be expressed as 
$$ 
f(z)=z+z(z-\sigma)u(z), 
$$
where $\sigma=\s(f)$ is a point in $D_{\rho/2}$ and $u(z)=u_f(z)$ is a non-zero 
holomorphic function defined in a neighbourhood of $\overline D_\rho$. 
Moreover $\s(f_0)=0$, $u_{f_0}(z)=(f_0(z)-z)/z^2$, 
$e^{2 \pi \alpha(f)}=1-\s(f)u_f(0)$, hence 
$\s(f)= - 2\pi i \alpha(f) (1+O(||f-f_0||))$, where 
$||\cdot||$ denotes the sup-norm on $\overline D_\rho$  and 
$f \mapsto \s(f)$, $f \mapsto u_f(z)$ (with $\Dom(u_f)=D_\rho$ fixed) 
are continuous.  
\endproclaim

Taking $\rho$ and $\N$ small, we may assume  that $\rho<1/4$ and  
$|u_f(z)-1|<1/2$ on $D_\rho$.  
We will simply write $\s$ and $u(z)$ if there is no confusion about $f$.  
Note that $0$ and $\s$ are the only fixed points of $f$ in 
$\overline D_\rho$.  

Let us introduce a new coordinate $w \in \C$ by 
$$ z = \t_\s (w) \equiv  \frac \s {1-e^{\s w}}. $$ 
And define the map $F(w)=F_{f}(w)$ by 
$$
F(w) = w - \frac 1\s 
\log \left( 1- \frac {\s u(z)}{1+zu(z)} \right) \quad \text{ with } z=\t_\s(w) 
\tag{4.??}$$
and 
$$T_\s(w)=w+\frac{2 \pi i}\s .$$
Here $F(w)$ is defined for $w$ such that $\t_\s(w) \in D_\rho$, hence 
$|\s u(z)/(1+zu(z))| \leq 1/2$, 
and (???) defines a single-valued function using the branch of logarithm with 
$-\pi <\Im \log (\cdot) \leq \pi$.  


\remark{Remark} This coordinate change has the following meaning:  
First, introduce a new coordinates $\zeta$ by 
$\exp(2\pi i \zeta) = \frac z{z-\s}. $
The M\"obius transformation $z \mapsto z/(z-\s)$ sends the fixed points $0$ 
and $\s$ to $0$ and $\infty$; 
hence $\zeta \mapsto z$ is a universal covering 
map from $\C$ to $\CC-\{0, \s\}$ with the covering transformation 
$\zeta \mapsto \zeta+1$.  It can be checked by a computation that $f$ can be
formally ``lifted'' to the map in $\zeta$-coordinate 
$$
\zeta \mapsto \zeta +
\frac 1{2\pi i} \log \left( 1- \frac {\s u(z)}{1+zu(z)} \right), 
$$
which resembles the translation 
$\zeta \mapsto \zeta - \s/2 \pi i $, when $z\sim 0$, $u(z)\sim 1$ and $\s \sim 0$.  

So we finally introduce a coordinate $\  w = -2\pi i \zeta / \s \ $, which 
coincides with the previous definition, and now the map resembles $w \mapsto w+1$.  
Then the covering transformation of the universal covering map $w \to z$ 
is 
$$T_\s(w)=w+\frac{2 \pi i}\s . $$
\endremark 

\proclaim{Lemma 4.4} {\rm (Properties of $F$, $\t_\s$ and $T_\s$)}
\newline 
(i) For $w, w' \in \C$, $\t_\s(w)=\t_\s(w')$ if and only if $w'=T_\s^n(w)$ for 
some $n \in \Z$.  $\t_\s(w) \to 0$ as $\Im \s w \to =\infty$, and 
$\t_\s(w) \to \s$ as $\Im \s w \to -\infty$.  
\newline   
(ii) There exists $R_0>0$ such that if $w \in \C - \cup _{n \in \Z} B_n(\s)$, 
where 
$B_n(\s) = \{w\in \C| \ |w-2\pi i /\s|<R_0/2 \ \}$, 
then  $\t_\s(w) \in D_\rho$ 
hence (???) is well-defined and satisfies
$|F(w)-(w+1)|<\frac 14$, $|F'(w)-1|< \frac 12$.  
\newline
(iii) $f \circ \t_\s = \t_\s \circ F$  and  $T_\s \circ F = F \circ T_\s$.  
\newline
(iv) $\t_\s(w) \to \t_0(w)$ as $ \s \to 0$  on $\{...\}$.  
$F_f(w)  \to F_0(w)$ as $f \to f_0$ unif on $\C-\cup B_n(\s)$.

\endproclaim 



\bigskip
\subheading{3.  Fatou coordinates for $f \in \N$}

Suppose that $\Re (-\frac {2\pi i}\s) >2R_0+2$ or $\s=0$.  Define 
$$\Q^+_\s=\Q(R_0, -R_0-\frac{2\pi i}\s), \ 
\Q^-_\s=\Q(R_0+\frac{2\pi i}\s, -R_0)=T_\s\Q^+_\s \ \text{ for } 
\s \neq 0, $$
$$\Q^+_0=\Q(R_0, +\infty), \ 
\Q^-_0=\Q(-\infty, -R_0).  $$
Then $F=F_f$ satisfies the condition in Lemma , and we have 

\proclaim{Lemma} Let $z^+_0 \in \t_0(\Q^+_0)$

If $f\in \N$ and $f'(0)=e^{2\pi i \a}$ with $\a \in W_r$, then there exist 
Fatou coordinates $\Phi_+$ for $F_f|_{\Q^+_\s}$ with base point $w_+$ and 
$\Phi_-$ for $F_f|_{\Q^-_\s}$ with base point $w_-$.  

$\Phi_+ \circ \Phi_-^{-1}$ is defined in $\Phi_{-,f}(\Q^+_\s \cap \Q^-_\s)$ and 
extends to regions $\{z|\ \Im z > \eta \}$ and $\{z|\ \Im z < \eta'\}$  
as a holomorphic map which commutes with $T$.  

Moreover $(f, z_+, z_-)\to (\Phi_+,\Phi_-)$ is continuous
So is $\Phi_+ \circ \Phi_-^{-1}$.  
\endproclaim

\definition{Definition} 
$\Phi_+$ (resp. $\Phi_-$) is called the {\it forward} (resp. {\it backward}) 
{\it Fatou coordinate} of $F$.  $\Phi_+ \circ \Phi_-^{-1}$ is called 
the {\it Ecalle transformation} (or {\it horn map}).  
$S_+$ $S_-$, $\Cal C^+$...
\enddefinition


$T_\s(w)=w+\frac{2 \pi i}\s$ 

$$\tR f(z)=\Phi_- \circ T_\s \circ \Phi_-^{-1}$$
on $\Phi_-(\Q_{-,\s} \cap \Q_{+,\s})$

\endcomment 











